CLIPC8: Face liveness detection algorithm based on image-text pairs and contrastive learning

Face recognition technology is widely used in the financial field, and various types of liveness attack behaviors need to be addressed. Existing liveness detection algorithms are trained on specific training datasets and tested on testing datasets, but their performance and robustness in transferring to unseen datasets are relatively poor. To tackle this issue, we propose a face liveness detection method based on image-text pairs and contrastive learning, dividing liveness attack problems in the financial field into eight categories and using text information to describe the images of these eight types of attacks. The text encoder and image encoder are used to extract feature vector representations for the classification description text and face images, respectively. By maximizing the similarity of positive samples and minimizing the similarity of negative samples, the model learns shared representations between images and texts. The proposed method is capable of effectively detecting specific liveness attack behaviors in certain scenarios, such as those occurring in dark environments or involving the tampering of ID card photos. Additionally, it is also effective in detecting traditional liveness attack methods, such as printing photo attacks and screen remake attacks. The zero-shot capabilities of face liveness detection on five public datasets, including NUAA, CASIA-FASD, Replay-Attack, OULU-NPU and MSU-MFSD also reaches the level of commercial algorithms. The detection capability of proposed algorithm was verified on 5 types of testing datasets, and the results show that the method outperformed commercial algorithms, and the detection rates reached 100% on multiple datasets. Demonstrating the effectiveness and robustness of introducing image-text pairs and contrastive learning into liveness detection tasks as proposed in this paper.

==> section/03_00_model.tex <==
%Fine-Grained Hierarchical Detection and Localization Network
%% if you use it as adj then you need to write fine-grained something
%\input{section/figure_table_latex/figure_architecture}
\Section{CLIPC8}
\label{sec:method}
\SubSection{Image Encoder} \label{sec_image_encoder}
This article employs the Vision Transformer (ViT) as the Image Encoder, with Fig.~\ref{figure_vit_model} illustrating the architecture and processing flow of the ViT. Images of arbitrary resolution \((h, w)\) are resized to a fixed resolution (M,M), and subsequently segmented into smaller image patches of resolution (c,c), according to the specified model parameters. The number of these segmented image patches, \( X_i \), denoted as \( N \), can be calculated using Equation (1):
\begin{equation}
	N = \frac{M \times M}{c^2}
\end{equation}

A trainable linear projection layer E maps N image patches \( X_i \), where $i \leq N$
, to an embedding layer, integrating classification information \( X_class \) with the image encoding to enable the model to discern and assimilate commonalities and differences between various categories, culminating in the necessity of appending positional labels \( P_pos \) to preserve the positional information of the images.We have:
\begin{equation}
	P_E = [X_{\text{class}}, X_E, X_1, X_2, \ldots, X_N] + P_{\text{pos}}
\end{equation}

A Transformer module is composed of a Multi-head Self-Attention layer (MSA) and a Multi-Layer Perceptron (MLP), with Layer Normalization (LN) applied to normalize the input data along the feature dimension. The output of \( l_th \) layer can be expressed in the following manner:
\begin{equation}
	y^l = \text{MSA}(\text{LN}(P^l)) + P^l
\end{equation}
\begin{equation}
	P^{(l+1)} = \text{MLP}(\text{LN}(y^l)) + y^l
\end{equation}

Here, \( P^l \) denotes the input to the \( l_th \) layer encoder, and \(y^l\)represents the intermediate variable.
\input{section/figure_table_latex/figure_cvit_model}

\SubSection{The CLIPC8 Method} \label{sec_clipc8_method}
This paper introduces the CLIPC8 methodology, a liveness detection approach based on image-text pair training. Utilizing the pretrained parameters of the ViT-L/14 model from CLIP, the method is trained on the CLASS-8 dataset. The goal is to exploit the supervisory signals inherent in natural language to train an image classification model. The training yields not only visual features but also multimodal features beneficial for transfer learning across different datasets. Image features \(I\) are obtained through the image encoding layer constructed by ViT, and text features \(T\) through the text encoding layer composed of Transformers. The cosine similarity \(S\) between text and image features is computed, followed by the application of a normalized exponential function (Softmax) to convert the network output into category probabilities \(C\). The highest-scoring category is deemed the current class. As introduced in Section 2, of the eight categories, (a) "Normal facial photographs captured using cameras of devices like smartphones or tablets" is classified as a genuine category, while the remaining seven are categorized under live attacks. The classification process is represented by the following formula:

\begin{equation}
	C = \text{softmax}(\text{cosine\_similarity}(I, T))
\end{equation}
\begin{equation}
	S = \text{cosine\_similarity}(I, T) = \frac{I \cdot T}{\| I \|_2 \cdot \| T \|_2}
\end{equation}
\begin{equation}
	C_i = \text{softmax}(S_i) = \frac{e^{S_i}}{\sum_{j=1}^{8} e^{S_j}}
\end{equation}
\begin{equation}
	L = \text{MAX}(C_i) = \left\{ \begin{array}{ll}
		Real, & \text{if}\ i=\text{index}(Real) \\
		Fake, & \text{if}\ i\neq\text{index}(Real)
	\end{array} \right.
\end{equation}

In this study, \(L\) denotes the final classification, with $1 \leq i \leq 8$ corresponding to the number of categories in the CLASS-8 dataset, and \(C_i\)Ci representing the category probability of each classification. When the highest scoring \(i\) equals the label number of a genuine human in the sample, the algorithm determines it as a real human; otherwise, it is identified as a live attack.

Fig.~\ref{figure_Contrastive_Learning} illustrates the training process of the CLIPC8 algorithm. During the training phase, the concept of contrastive learning is utilized to compare positive samples (images and corresponding classification texts) with negative samples (images and texts of different classifications). The ViT structure is employed as the backbone network. The model processes image-text pairs as inputs and computes their similarity in the vector space. The CrossEntropyLoss function encourages higher scores for positive samples and lower scores for negative samples. Through contrastive learning, the CLIPC8 model learns a shared representation linking images and texts. 
\input{section/figure_table_latex/figure_Contrastive}
Fig.~\ref{figure_liveness_detection} shows the input and output of the model during the prediction phase. To determine whether the subject is a real human or a live attack, the CLIPC8 model receives an image along with eight sets of text classification prompts. The model calculates the similarity between the input image and each classification prompt, with the highest similarity indicating the predicted category.
\input{section/figure_table_latex/figure_liveness_detection}

